Bulgeless disks, dark galaxies, inverted color gradients, and other expected phenomena at higher z. The chromatic surface brightness modulation (CMOD) effect

Since the k correction depends on the spectral energy distribution (SED) of a galaxy, any high-z galaxy with a spatially non-homogeneous SED will experience a spatially varying relative dimming or brightening in addition to the pure distance effect. The morphology of galaxies will therefore change with z. For instance, an early spiral galaxy observed in the V band would show a prominent bulge at z=0, whereas, if at z=1, the V filter probes the rest-frame near-UV where the bulge is faint and the disk relatively brighter, thus the galaxy may appear as bulgeless. For galaxies with strong nebular emission, an additional effect is that the shifting of strong nebular features in or out of filters will result in a non-monotonous color evolution with z. Hence, unlike the effects of distance, cosmological surface brightness dimming, and gravitational lensing, which are all achromatic, the fact that most galaxies have a spatially varying SED leads to a chromatic surface brightness modulation (CMOD) with z. While the CMOD effects are in principle easy to grasp, they affect the characterization of galaxies in a complex fashion. Properties such as the bulge-to-disk ratio, Sersic exponent, effective radius, radial color gradients, and stellar mass determinations from SED fitting will depend on z, the filters employed, and the rest-frame 2D SED patterns in a galaxy, and will bias results inferred on galaxy evolution across cosmic time (e.g., the evolution of the mass-size, bulge-SMBH, and Tully-Fisher relation), if these effects are not properly taken into account. In this article we quantify the CMOD effects for idealized galaxies built from spectral synthesis models and from galaxies with observed integral field spectroscopy, and we show that they are significant and should be taken into account in studies of resolved galaxy properties and their evolution with z. (abridged)

==> References.tex <==
% References.tex
\begin{thebibliography}{}
\baselineskip=0ex
\bibitem[Abraham et al.(1996)]{Abraham96}Abraham, R.G., van den Bergh, S., Glazebrook, K. et al. 1996, ApJS 107, 1
\bibitem[Amor\'in et al.(2012)]{Amorin2012}Amor\'in, R., P\'erez-Montero, E., V\'ilchez, J. M., Papaderos, P., 2012, ApJ, 749, 185A
\bibitem[Anders \& Fritze-v. Alvensleben(2003)]{AFvA03}Anders, P. \& Fritze von Alvensleben 2003, A\&A 401, 1063
\bibitem[Armus et al.(1987)]{Armus87}Armus, L., Heckman, T. \& Miley, G. 1987, AJ, 94, 831
\bibitem[Atek et al.(2011)]{Atek11}Atek, H., Siana, B., Scarlata, C. et al. 2011, ApJ 743, 121
\bibitem[Atek et al.(2022)]{Atek22}Atek, H., Furtak, L.J., Oesch, P. et al. 2022, MNRAS, 511, 4464
\bibitem[Bacon et al.(2014)]{Bacon14}Bacon, R., Vernet, J., Borisova, E., et al. 2014, The Messenger, 157, 13
\bibitem[Balcells \& Peletier(1994)]{BP94}Balcells, M. \& Peletier, R.F. 1994, AJ, 107, 135
\bibitem[Barden et al.(2008)]{Barden08}Barden, M., Jahnken, K. \& H\"au\ss ler, B. 2008, ApJ Suppl. 175, 105  % FERENGI
\bibitem[Barsanti et al.(2021)]{Barsanti21}Barsanti, S., Owers, M.S., McDermid, R.M. et al.  2021, ApJ 906, 100B
\bibitem[Beare et al.(2014)]{Beare14}Beare, R., Brown, M.J.I. \& Pimbblet, K. 2014, ApJ, 797, 104
\bibitem[Belfiore et al.(2018)]{Belfiore18}Belfiore, F., Maiolino, R., Bundy, K. et al. 2018, MNRAS, 477, 3014
\bibitem[Bergvall \& Olofsson(1986)]{BO86}Bergvall, N. \& Olofsson, K. 1986, A\&AS, 64, 469
\bibitem[Bergvall \& \"Ostlin(2002)]{BO02}Bergvall, N. \& \"Ostlin, G., 2002, A\&A, 390, 891
\bibitem[Bergvall et al.(2006)]{Bergvall06}Bergvall, N., Zackrisson, E., Andersson B.-G. et al. 2006, A\&A, 448, 513
\bibitem[Bernardi et al.(2003)]{Bernardi03}Bernardi, M., Sheth, R.K., Annis, J. et al. 2003, AJ, 125, 1817
\bibitem[Bernl\"ohr(1993)]{Bernlohr93}Berln\"ohr. K. 1993, A\&A, 268, 25
\bibitem[Bershady et al.(2000)]{Bershady00}Bershady, M., Jangren, A. \& Conselice, C. 2000, AJ, 119, 2645
\bibitem[Bicker \& Fritze-v. Alvensleben(2005)]{BFvA05}Bicker, J. \& Fritze-v. Alvensleben, U. 2005, A\&A 443, L19
\bibitem[Bicker et al.(2004)]{Bicker04}Bicker, J., Fritze-v. Alvensleben, U., M\"oller, C.S. \& Fricke, K.J. 2004, A\&A 413, 37  % k+e corrections
\bibitem[{{Binette} {et~al.}(1994){Binette}, {Magris}, {Stasi{\'n}ska}, \& {Bruzual}}]{bin94} {Binette}, L., {Magris}, C.~G., {Stasi{\'n}ska}, G., \& {Bruzual}, A.~G. 1994, \aap, 292, 13
\bibitem[Bittner et al.(2017)]{Bittner17}Bittner, A., Gadotti, D.A., Elmegreen, B.G. et al. 2017, MNRAS, 471, 1070
\bibitem[Bittner et al.(2020)]{Bittner20}Bittner, A., S\'anchez-Bl\'azquez, P. Gadotti, D.A. et al. 2020, A\&A 643, 65
\bibitem[Bizzocchi et al.(2014)]{Bizzocchi14}Bizzocchi, L., Filho, M.E., Leonardo, E. et al. 2014, ApJ, 782, 22
\bibitem[Blanton et al.(2003)]{Blanton03}Blanton, M.R., Brinkmann, J., Csabal, I. et al. 2003, AJ, 125, 2348
\bibitem[Blanton \& Roweis(2007)]{BR07}Blanton, M.R. \& Roweis, S. 2007, AJ, 133, 734  % KCORRECT
\bibitem[Bohlin et al.(1991)]{Bohlin91}Bohlin, H.C., Cornett, R.H., Hill, J.K. et al. 1991, ApJ, 368, 12
\bibitem[B\"ohm et al.(2004)]{Boehm04}B\"ohm, A., Ziegler, B.L., Saglia, R.P. et al. 2004, A\&A, 420, 97
\bibitem[Bournaud et al.(2007)]{Bournaud07} Bournaud, F., Elmegreen, B. G., Elmegreen, D. M., 2007, ApJ, 670, 237
\bibitem[Boyett et al.(2022)]{Boyett22}Boyett, K., Mascia, S., Pentericci, L. et al. 2022, ApJL, submitted (arXiv:2207.13459)
\bibitem[Brammer et al.(2008)]{Brammer08}Brammer, G.B., van Dokkum, P.G. \& Coppi, P. 2008, ApJ, 686, 1503
\bibitem[Bretonnière et al.(2022)]{Bretonniere22}Bretonni\`ere, H., Kuchner, U., Huertas-Company, M. et al. 2022, A\&A, in press (arXiv:2209.12907)
\bibitem[Breda \& Papaderos(2018)]{BP18}Breda, I. \& Papaderos, P. 2018, A\&A 614, 48 \tref{(BP18)}
\bibitem[Breda(2019)]{B19}Breda, I., 2019, PhD Thesis, University of Porto
%\bibitem[Breda et al.(2019)]{Breda19}Breda, I., Papaderos, P., Gomes, J.M., Amarantidis, S. 2019, A\&A, 632, A128
\bibitem[Breda et al.(2020a)]{Breda20a}Breda, I., Papaderos, P., Gomes, J.M. et al. 2020a, A\&A, 635, A177
\bibitem[Breda et al.(2020b)]{Breda20b}Breda, I., Papaderos, P. \& Gomes, J.M. 2020b, A\&A, 640A, 20B
\bibitem[Breda et al.(2022)]{Breda22}Breda, I. et al. 2022, A\&A, 663, 29
\bibitem[Breda \& Papaderos(2023)]{BP23}Breda, I. \& Papaderos, P. 2023, A\&A, 669, A70 
\bibitem[Brinchmann et al.(2004)]{Bri04} Brinchmann, J., Charlot, S., White, S. D. M. et al. 2004, MNRAS, 351, 1151
\bibitem[Brinchmann(2022)]{Brinchmann22}Brinchmann, J. 2022, MNRAS, submitted (arXiv:2208.07467)
\bibitem[Bruzual \& Charlot(2003)]{BruCha03} Bruzual, G. \& Charlot, S., 2003, MNRAS, 344, 1000
\bibitem[Buitrago et al.(2008)]{Buitrago08}Buitrago, F., Trujillo, I., Conselice, C. J., et al. 2008, ApJ, 687, L61
\bibitem[Buitrago et al.(2013)]{Buitrago13}Buitrago, F., Trujillo, I., Conselice, C.J. \& H\"au\ss ler, B. 2013, MNRAS, 428, 1460
\bibitem[Buitrago et al.(2017)]{Buitrago17}Buitrago, F., Trujillo, I., Curtis-Lake, E. et al. 2017, MNRAS, 466, 4888
\bibitem[Buta \& Combes(1996)]{ButaCombes96}Buta, R. \& Combes, F. 1996, Fund. Cosmic Physics, 17, 95
\bibitem[Butcher \& Oemler(1978)]{BO78}Butcher, H. \& Oemler, A., Jr. 1978, ApJ, 226, 559
\bibitem[Butcher \& Oemler(1984)]{BO84}Butcher, H. \& Oemler, A., Jr. 1984, ApJ, 285, 426
\bibitem[Byler et al.(2017)]{Byler17}Byler, N., Dalcanton, J.J., Conroy, C., Johnson, B.D. 2017, ApJ, 840, 44
\bibitem[Calzetti et al.(2000)]{Calzetti00}Calzetti D., Armus L., Bohlin R.C. et al. 2000. ApJ 533, 682
\bibitem[Catal\'an-Torrecilla et al.(2017)]{CatT17}Catal\'an-Torrecilla, C., Gil de Paz, A., Castillo-Morales, A. et al. 2017, ApJ, 848, 87
\bibitem[Cardamone et al.(2009)]{Cardamone09}Cardamone, C., Schawinski, K., Sarzi, M. et al. 2009, MNRAS, 399, 1191
\bibitem[Cardelli et al.(1989)]{Cardelli89}Cardelli J. A., Clayton G. C., Mathis J. S., 1989, ApJ, 345, 245
\bibitem[Cattaneo et al.(2009)]{Cattaneo09}Cattaneo, A., Faber, S. M., Binney, J., Dekel, A., Kormendy, J. et al. 2009, Nature, 460, 213
\bibitem[Charlot \& Longhetti(2001)]{ChaLon01} Charlot, S, \& Longhetti, M. 2001, MNRAS, 323, 887
\bibitem[Chamba et al.(2022)]{Chamba22}Chamba, N., Trujillo, I. \& Knappen, J.H. 2022, A\&A, 667, A87
\bibitem[Chevallard \& Charlot(2016)]{CC16}Chevallard J. \& Charlot S., 2016, MNRAS, 462, 1415
\bibitem[Chilingarian et al.(2010)]{Chil10}Chilingarian, I.V., Melchior, A.-L., Zolotukhin, I.Yu. 2010, MNRAS, 405, 1409
\bibitem[Cid Fernandes et al.(2005)]{Cid05} Cid Fernandes, R., Mateus, A., Sodr\'{e}, L., Stasi\'{n}ska, G., Gomes, J. M., 2005, MNRAS, 358, 363
\bibitem[Cid Fernandes et~al.(2011)]{Cid11}Cid Fernandes, R., Stasi{\'n}ska, G., Mateus, A. et al. 2011, \mnras, 413, 1687
\bibitem[Cirasuolo et al.(2020)]{Cirasuolo20}Cirasuolo, M., Fairley, A., Rees, P., et al. 2020, The Messenger, 180, 10
\bibitem[Coleman et al.(1980)]{Coleman80}Coleman, G.D., Wu, C.-C. \& Weedman, D.W. 1980, ApJS, 43, 393C   % k-corrections
\bibitem[Comer\'on et al.(2012)]{Comeron12}Comer\'on, S., Elmegreen, B.G., Salo, H. et al. 2012, ApJ 759, 98
\bibitem[Conselice(2003)]{Conselice03}Conselice, C. 2003, ApJS, 147, 1
\bibitem[Conselice et al.(2005)]{Conselice05}Conselice, C.J., Blackburne, J.A. \& Papovich, C. 2005, ApJ, 620, 564
\bibitem[Conselice et al.(2008)]{Conselice08}Conselice, C.J., Rajgor, S \& Myers, R. 2008, MNRAS, 386, 909
\bibitem[Conselice et al.(2011)]{Conselice11}Conselice, C.J., Bluck, A.F.L., Ravindranath, S. et al. 2011, MNRAS, 417, 2770
\bibitem[Conselice(2014)]{Conselice14}Conselice, C.J. 2014, ARA\&A, 52, 291
\bibitem[Comer\'on et al.(2010)]{Comeron10}Comer\'on, S., Knapen, J. H., Beckman, J. E. et al. 2010, MNRAS, 402, 246
\bibitem[Combes(2000)]{Combes00}Combes, F. 2000, in {\sl Building Galaxies; from the Primordial Universe to the Present}, Proceedings of the XIXth Rencontres de Moriond held at Les Arcs, March 13-20, 1999. F. Hammer, T.X. Thuan, V. Cayatte et al. (eds.). World Scientific Publishing Co. p.413
\bibitem[Contardo et al.(1998)]{Contardo98}Contardo, G., Steinmetz, M. \& Fritze-von Alvensleben 1998, ApJ, 507, 497
\bibitem[Costantin et al.(2021)]{Costantin21}Costantin, L., P\'erez-Gonz\'alez, P.G., M\'endez-Abreu, J. et al. 2021, ApJ, 913, 125
\bibitem[Courteau et al.(1996)]{Courteau96}Courteau, S., de Jong, R.S., Broeils, A.H. 1996, ApJ 457, L73
\bibitem[Cowie et al.(1996)]{Cowie96}Cowie, L.L., Songaila, A., Hu, E. M. \& Cohen, J. G. 1996, AJ, 112, 839
\bibitem[Croton et al.(2006)]{Croton06}Croton, D.J., Springel, V., White, S.D.M. et al. 2006, MNRAS, 365, 11
\bibitem[Davies et al.(1987)]{Davies87}Davies, R.L., Burstein, D., Dressler, A. et al. 1987, ApJS 64, 581
\bibitem[de Lorenzo-C\'aceres et al.(2019)]{dLC19}de Lorenzo-Cáceres, A.; Méndez-Abreu, J.; Thorne, B.; Costantin, L. 2019, MNRAS 484, 665
\bibitem[de Jong \& van der Kruit(1994)]{dJvK94}de Jong, R.S. \& van der Kruit, P.C. 1994, A\&A Suppl. 104, 451
\bibitem[de Jong(1996a)]{deJong96a}de Jong, R.S. 1996a, A\&A Suppl. 118, 557
\bibitem[de Jong(1996b)]{deJong96b}de Jong, R.S. 1996b, A\&A 313, 377
\bibitem[Dekel et al.(2009)]{Dekel09}Dekel, A., Birnboim, Y., Engel, G., et al. 2009, Nature, 457, 451
\bibitem[Dekel \& Burkert(2014)]{DekelBurkert14}Dekel, A. \& Burkert, A. 2014, MNRAS, 438, 1870
\bibitem[Dey et al.(2019)]{Dey19}Dey A. et al., 2019, AJ, 157, 168
\bibitem[Di Matteo et al.(2005)]{DMSH05}Di Matteo, T., Springel, V. \& Hernquist, L. 2005, Nature, 433, 604 
\bibitem[dos Reis et al.(2020)]{dosReis20}dos Reis, S., Buitrago, F., Papaderos, P. et al. 2020, A\&A, 634, 11D
\bibitem[Dressler(1980)]{Dressler80}Dressler, A. 1980, ApJ, 236, 351                    % morphology-density
\bibitem[Dressler et al.(1987)]{Dressler87}Dressler, A., Lynden-Bell, D., Burstein, D., et al. 1987, ApJ, 313, 42
\bibitem[Driver et al.(1995)]{Driver95}Driver, S.P., Windhorst, R.A., Ostrander, E.J. et al. 1995, ApJ, 449, L23
%\bibitem[Drory \& Fisher(2007)]{DroFis07}Drory, N. \& Fisher, D., 2007, ApJ, 664, 640
\bibitem[Duc \& Mirabel(1994)]{DM94}Duc, P.-A. \& Mirabel, I.F. 1994, A\&A, 289, 83 % Arp 105
\bibitem[Duc et al.(2015)]{Duc15}Duc, P.-A., Cuillandre, J.C., Karabal, E. et al. 2015, MNRAS, 446, 120
\bibitem[Dwek \& Arendt(2020)]{DA2020}Dwek, E. \& Arendt, R.G. 2020, ApJ 901, 36
% Star formation is boosted (and quenched) from the inside-out: radial star formation profiles from MaNGA
\bibitem[Ellison et al.(2018)]{Ellison18}Ellison, S.L., S\'anchez, S.F., Ibarra-Medel, H. et al. 2018, MNRAS, 474, 2039
\bibitem[Elmegreen et al.(2007)]{Elmegreen07}Elmegreen, D.M., Elmegreen, B.G., Ravindranath, S., Coes, D.A. 2007, ApJ, 658, 763
\bibitem[Elmegreen et al.(2008)]{Elm08} Elmegreen, B.G., Bournaud F., Elmegreen D.M., 2008, ApJ, 688, 67
\bibitem[Er et al.(2018)]{Er18}Er, X., Hoekstra, H., Schrabback, T. et al. 2018, MNRAS 476, 5645
\bibitem[Fang et al.(2013)]{Fang13}Fang, J. J., Faber, S. M., Koo, D. C. \& Dekel, A. 2013, ApJ, 776, 63
\bibitem[Fensch et al.(2016)]{Fensch16}Fensch, J., Duc, P.-A., Weilbacher, P. et al. 2016, A\&A, 585, A79
\bibitem[Ferguson \& Binggeli(1994)]{FB94}Ferguson, H.C. \& Binggeli, B. 1994, A\&A Review, 6, 67
\bibitem[Fetherolf et al.(2023)]{Fetherolf23}Fetherolf, T., Reddy, N.A., Shapley, A.E. et al. 2023, MNRAS, 518, 42
\bibitem[Fielder et al.(2022)]{Fielder22}Fielder, C.E., Andrews, B.H., Newman, J.A., Salim, S. 2022, MNRAS, submitted (arXiv.2212.03263)
\bibitem[Fioc \& Rocca-Volmerange(1997)]{FRV97}Fioc, M., \& Rocca-Volmerange, B. 1997, A\&A, 326, 950
\bibitem[Fiore et al.(2022)]{Fiore22}Fiore, F., Ferrara, A., Bischetti, M., Feruglio, C \& Travascio, A. 2022, ApJL, submitted (arXiv:2211.08937)
%\bibitem[Fudamoto et al.(2022)]{Fudamoto22}Fudamoto, Y., Inoue, A.K. \& Sugahara, Y. 2022, ApJL, 938, 24
\bibitem[Garc\'ia-Benito et al.(2015)]{GB15CALIFA}Carc\'ia-Benito, R., Zibetti, S., S\'anchez, S.F. et al. 2015, A\&A, 576. A135
\bibitem[Gavazzi et al.(2002)]{Gavazzi02}Gavazzi, G., Bonfanti, C., Sanvito, G. et al. 2002, ApJ 576, 135     % delayed exp. SFHs a la Sandage
\bibitem[Gallagher et al.(1984)]{Gallagher84}Gallagher, J.S. III, Hunter, D.A. \& Tutukov, A.V. 1984, ApJ 284, 544
\bibitem[Gadotti et al.(2020)]{Gadotti20}Gadotti, D.A., Bittner, A., Falc\'on-Barroso, J. et al. 2020, A\&A 643, 14
\bibitem[Ganda et al.(2007)]{Ganda07}Ganda, K., Peletier, R.F., McDermid, R.M., et al. 2007, MNRAS, 380, 506
\bibitem[Genzel et al.(2014)]{Genzel14}Genzel, R. et al. 2014, ApJ 785, 75
\bibitem[Gil de Paz et al.(2002)]{GdP02}Gil de Paz, A., Silich, S.A., Madore, B.F. et al. 2002, ApJ, 573, L101
\bibitem[Gil de Paz et al.(2003)]{GdP03}Gil de Paz, A., Madore, B.F., \& Pevunova, O. 2003, ApJS, 147, 29
\bibitem[Gomes et al.(2016)]{GP16-ETGs}Gomes, J.M., Papaderos, P., Kehrig, C. et al. 2016, A\&A, 588, 68
\bibitem[Gomes \& Papaderos(2016)]{GP16-RY}Gomes, J.M. \& Papaderos, P., 2016, A\&A, 594, A49 % RY
\bibitem[Gomes \& Papaderos(2017)]{GP17}Gomes, J.M. \& Papaderos, P., 2017, A\&A, 602, A63    % FADO
\bibitem[Goto et al.(2003)]{Goto03}Goto, T., Chisato, Y., Yutaka, F. et al. 2003, MNRAS, 346, 601
\bibitem[Guiderdoni \& Rocca-Volmerange(1987)]{GRV87}Guiderdoni, B. \& Rocca-Volmerange, B. 1987, A\&A, 186, 1
\bibitem[Guseva et al.(2001)]{Guseva01}Guseva, N.G., Izotov, Y. I., Papaderos, P. et al. 2001, A\&A, 378, 756
\bibitem[Guseva et al.(2004)]{Guseva04}Guseva, N.G., Papaderos, P., Izotov, Y.I., Noeske, K.G., Fricke, K.J. 2004, A\&A, 421, 519
\bibitem[Guy et al.(2022)]{Guy22}Guy, L.P., Cuillandre, J.-C., Bachelet, E. et al. 2022 (arxiv.org:2201.03862)
\bibitem[H\"au\ss ler et al.(2013)]{H13}H\"au\ss ler, B., Bamford, S.P., Vika, M. et al. MNRAS 430, 330
\bibitem[Hayes et al.(2007)]{Hayes07}Hayes, M., \"Ostlin, G., Atek, H., Kunth, D. 2007, MNRAS, 382, 1465
\bibitem[Heckman \& Best(2014)]{HeckmanBest14}Heckman, T.M. \& Best, P.N. 2014, ARA\&A, 52, 589
\bibitem[Hester et al.(2010)]{Hester10}Hester, J.A., Seibert, M., Neill, J.D et al. 2010, ApJL, 716, 14  % IC3418
\bibitem[Hogg et al.(2002)]{Hogg02}Hogg., D.W., Baldry, I.K., Blanton, M.R., Eisenstein, D.J. 2002, arXiv:0210394v1  % discussion k-correction
\bibitem[Huertas-Company et al.(2015)]{HC15}Huertas-Company, M., P\'erez-Gonz\'alez, P.G., Mei, S. et al. 2015, ApJ, 809, 95
\bibitem[Huertas-Company et al.(2020)]{HC20}Huertas-Company, M., Guo, Y., Ginzburg, O. et al. 2020, MNRAS, 499, 814
\bibitem[Huchra(1977)]{Huchra77}Huchra, J. P. 1977, ApJ, 217, 928
\bibitem[Humason et al.(1956)]{Humason56}Humason, M.L., Mayall, N.U., Sandage, A.R., 1956, AJ, 61, 97
\bibitem[Inami et al.(2022)]{Inami22}Inami, H., Algera, H., Schouws, S. et al. 2022, MNRAS, 515, 3126
\bibitem[Inayoshi et al.(2022)]{Inayoshi22}Inayoshi, K., Onoue,M., Sugahara, Y., Inoue, A.K., Ho, L.C. 2022, ApJL, submitted (arXiv:2204.09692)
\bibitem[Inoue \& Kamaya(2004)]{IK04}Inoue, A.K. \& Kamaya, H. 2004, MNRAS 350, 729
\bibitem[Inoue(2011)]{Inoue11}Inoue, A.K. 2011, MNRAS, 415, 2920
\bibitem[Izotov et al.(1997)]{Izotov97}Izotov, Y.I., Lipovetsky, V.A., Chaffee, F.H. et al. 1997, ApJ, 476, 698
\bibitem[Izotov et al.(2004)]{Izotov04}Izotov, Y.I., Papaderos, P., Guseva, N.G. et al. 2004, A\&A, 421, 539 % Tol 65+Tol1214-277
\bibitem[Izotov et al.(2006)]{Izotov06}Izotov, Y.I., Schaerer, D., Blecha, D. et al. 2006, A\&A, 459, 71     % SBS 0335-052
\bibitem[Izotov et al.(2011)]{Izotov11}Izotov, Y.I., Guseva, N.G., Thuan, T.X. 2011, ApJ, 728, 161
\bibitem[Johnston et al.(2012)]{Johnston12}Johnston, E.J., Arag\'on-Salamanca, A., Merrifield, M. R., Bedregal, A. G., 2012, MNRAS, 422, 2590
\bibitem[Johnston et al.(2017)]{Johnston17}Johnston, E. J., H\"au\ss ler, B., Arag\'on-Salamanca, A. et al. 2017, MNRAS, 465, 2317
\bibitem[Joseph \& Wright(1985)]{JosephWright85}Joseph, R.D. \& Wright, G. S. 1985, MNRAS, 214, 87
\bibitem[Kalinova et al.(2021)]{Kalinova21}Kalinova, V., Colombo, D., S\'anchez, S.F. et al. 2021, A\&A, 648A, 64K 
\bibitem[Kamath et al.(2020)]{Kamath20}Kamath, S., Meyers, J.E., Burchat, P.R. 2020, ApJ, 888, 23
\bibitem[Kauffmann et~al.(2003)]{Kauffmann03}Kauffmann, G., Heckman, T.~M., Tremonti, C., et al. 2003, MNRAS, 346, 1055
\bibitem[Kehrig et al.(2018)]{Kehrig18}Kehrig, C., V\'ilchez, J.M., Guerrero, M.A. et al. 2018, MNRAS, 480, 1081
\bibitem[Kennicutt(1989)]{Kennicutt89} Kennicutt, R.C., Jr. 1989, ApJ, 344, 685
\bibitem[Kennicutt et al.(2009)]{Kennicutt09}Kennicutt, R.C., Hao, C.-N., Calzetti, D. eet al. 2009, ApJ, 703, 1672
\bibitem[Kinney et al.(1996)]{Kinney96}Kinney, A., Calzetti, D., Bohlin, R.C. et al. 1996, ApJ 467, 38
\bibitem[Kotulla et al.(2009)]{Kotulla09}Kotulla, R., Fritze, U., Weilbacher, P. \&  Anders, P. 2009, MNRAS, 396, 462
\bibitem[Kormendy \& Kennicutt(2004)]{KorKen04} Kormendy, J. \& Kennicutt Jr, R. 2004, ARA\&A, 42, 603
\bibitem[Kormendy \& Ho(2013)]{KH13}Kormendy, J. \& Ho, L.C., 2013, ARA\&A, 51, 511
\bibitem[Kr\"{u}ger et al.(1995)]{Krueger95} Kr\"{u}ger, H., Fritze von Alvensleben, U. \& Loose, H.-H. 1995, A\&A, 303, 41
\bibitem[Kunth et al.(1988)]{Kunth88}Kunth, D., Maurogordato, S. \& Vigroux, L. 1988, A\&A, 204, 10 
\bibitem[Lassen et al.(2021)]{Lassen21}Lassen, A.E., Riffel, R., Chies-Santos, A.L. et al. 2021, MNRAS, 506, 3527
\bibitem[Larson et al.(1980)]{LarsonTinsleyCaldwell1980}Larson, R.B., Tinsley, B.M. \& Caldwell, C.N. 1980, ApJ, 237, 692
\bibitem[Leitherer et al.(1999)]{Lei99} Leitherer, C., Schaerer, D., Goldader, J.D., Gonz\'{a}lez-Delgado, R. M., Robert, C., Kune, D. F., de Mello, D. F., Devost, D. \& Heckman, T. M., 1999, ApJS, 123, 3 
\bibitem[Laurikainen et al.(2018)]{Laurikainen18}Laurikainen, E., Salo, H., Laine, J., Janz, J. 2018, A\&A 618, 34
\bibitem[Leitet et al.(2011)]{Leitet11}Leitet, E., Bergvall, N., Piskunov, N., Andersson B.-G., 2011, A\&A, 532, A107
\bibitem[Lequeux et al.(1979)]{Lequeux79} Lequeux J., Peimbert M., Rayo J. F., Serrano A., Torres-Peimbert S., 1979, A\&A, 80, 155L
\bibitem[Lilly et al.(1996)]{Lilly96}Lilly, S.J., Le Fevre. O., Hammer F., Crampton. D. 1996, ApJ, 460, L1
\bibitem[Liu et al.(2023)]{Liu23}Liu, D., F\"orster-Schreiber, N.M., Genzel, R. et al. 2023, ApJ, 942, 98
\bibitem[Llerena et al.(2023)]{Llerena23}Llerena, M., Amor\'in, R., Pentericci, L. et al. 2023, A\&A, in press (arxiv.org/pdf/2303.01536.pdf)
\bibitem[Loose \& Thuan(1986)]{LT86}Loose, H.-H. \& Thuan, T.X. 1986, in Star-Forming Galaxies and Related Objects, eds. D. Kunth, T.X. Thuan, \& T.T. Van 
(Paris: Editions Frontières), 73
\bibitem[Lotz et al.(2004)]{Lotz04}Lotz, J.M., Primack, J. \& Madau, P. 2004, AJ, 128, 163
\bibitem[Lumbreras-Calle et al.(2022)]{LC22}Lumbreras-Calle, A., L\'opez-Sanjuan, C., Sobral, D., Fern\'andez-Ontiveros, J.A., V\'ilchez, J.M. et al. 2022, A\&A, 668, A60
\bibitem[Madau et al.(1996)]{Madau96}Madau P., Ferguson, H.C., Dickinson, M.E. et al. 1996, MNRAS, 283, 1388
\bibitem[Madau \& Dickinson(2014)]{MD14}Madau, P. \& Dickinson, M. 2014, ARA\&A 52, 415
\bibitem[Mandelker et al.(2014)]{Mandelker14}Mandelker, N., Dekel, A., Ceverino, D. et al. 2014, MNRAS 443, 3675
\bibitem[Mandelker et al.(2017)]{Mandelker17}Mandelker, N., Dekel, A, Ceverino, D., et al. 2017, MNRAS 464, 635
\bibitem[Mannucci et al.(2001)]{Mannucci01}Mannucci, F., Basile F., Poggianti B. M. et al. 2001, MNRAS, 326, 745
\bibitem[Mart\'inez-Delgado et al.(2010)]{MD10}Mart\'inez-Delgado, D., Galbany, R.J., Crawford, K. et al. 2010, AJ, 140, 962
\bibitem[Maseda et al.(2014)]{Maseda14}Maseda, M.V., van der Wel, A., Rix, H.-W. et al. 2014, ApJ, 791, 17
\bibitem[Marino et al.(2018)]{Marino18}Marino, R.A., Cantalupo, S., Lilly, S.J. et al. 2018, ApJ, 859, 53
\bibitem[Martig et al.(2009)]{Martig09}Martig, M., Bournaud, F., Teyssier, R., Dekel, A. 2009, ApJ 707, 250
\bibitem[Matthee et al.(2022)]{Matthee22}Matthee, J., Mackenzie, R. Simcoe, R.A. et al. 2022, ApJ, submitted (arXiv:2211.08255)
\bibitem[Menacho et al.(2019)]{Menacho19}Menacho, V., \"Ostlin, G., Bik, A., et al. 2019, MNRAS, 487, 3183
\bibitem[Menacho et al.(2021)]{Menacho21}Menacho, V., \"Ostlin, G., Bik, A., et al. 2021, MNRAS, 506, 1777
\bibitem[M\'{e}ndez-Abreu et al.(2008)]{Men08} M\'{e}ndez-Abreu, J., Aguerri, J. A. L., Corsini, E. M. \& Simonneau, E., 2008, A\&A, 478, 353
\bibitem[M\'{e}ndez-Abreu et al.(2017)]{Men17} M\'{e}ndez-Abreu, J., Ruiz-Lara, T., S\'anchez-Menguiano, L. et al. 2017, A\&A 598, A32
\bibitem[Merlin et al.(2022)]{Merlin22}Merlin, E., Castellano, M., Bretonni\`ere, H. et al. 2022, A\&A, in press (arXiv:2209.12906)
\bibitem[Merritt et al.(2016)]{Merritt16} Merritt, A., van Dokkum, P., Abraham, R. \& Zhang, J. 2016, ApJ, 830, 62
\bibitem[Me\v{s}tri\'{c} et al.(2022)]{Mestric22}Me\v{s}tri\'{c}, U., Vanzella, E., Zanella, A. et al. 2022, MNRAS, 516, 3532
\bibitem[Micheva et al.(2017)]{Micheva17}Micheva, G., Oey, M.S., Jaskot, A.E. \& James, B.L. 2017, ApJ, 845, 165
\bibitem[Mobasher et al.(2015)]{Mobasher15}Mobasher, B., Dahlen, T., Ferguson, H. C., et al. 2015, ApJ, 808, 101
\bibitem[Morishita et al.(2019)]{Morishita19}Morishita, T., Abramson, L.E., Treu, T. et al. 2019, ApJ, 877, 141
\bibitem[Mosleh et al.(2017)]{Mosleh17}Mosleh, M., Tacchella, S., Renzini, A. et al. 2017, ApJ 837, 2
\bibitem[Muchotzky \& Scharf(1997)]{MS97}Muchotzky, R.F. \& Scharf, C.A. 1997, ApJ, 482, L13
\bibitem[Mulchaey \& Zabludoff(1998)]{MZ98}Mulchaey, J.S. \& Zabludoff, A.I. 1998, ApJ 496, 73
\bibitem[Nakajima \& Ouchi(2014)]{NO14}Nakajima, K. \& Ouchi, M. 2014, MNRAS, 442, 900
\bibitem[Nedkova et al.(2021)]{Nedkova21}Nedkova, K., H\"au\aa ler, B., Marchesini, D. et al. 2021, MNRAS, 506, 928
\bibitem[Nelson et al.(2022)]{Nelson22}Nelson, E.J., Suess, K.A., Bezanson, R. et al. 2022, arXiv:2208.01630
\bibitem[Neumann et al.(2017)]{Neumann17}Neumann, J., Wisotzki, L., Cloudhury, O. S., Gadotti, D. A., Walcher, C. J. et al. 2017, A\&A, 604, 30
\bibitem[Noeske et al.(2003)]{Noeske03}Noeske, K.G. Papaderos, P., Cair\'os, L.M., Fricke, K.J. 2003, A\&A, 410, 481
\bibitem[Noeske et al.(2007)]{Noeske07}Noeske, K.G., Faber, S.M., Weiner, B.J., et al. 2007, ApJL, 660, 47
\bibitem[Noguchi(1999)]{Noguchi99}Noguchi, M., 1999, ApJ, 514, 77
\bibitem[Nussbaumer \& Schmutz(1984)]{NussbaumerSchmutz84}Nussbaumer H. \& Schmutz W., 1984, A\&A, 138, 495
\bibitem[Oke \& Sandage(1968)]{OkeSandage68}Oke, J.B. \& Sandage, A. 1968, ApJ, 154, 21
\bibitem[\"Ostlin et al.(2003)]{Ostlin03}\"Ostlin, G., Zackrisson, E., Bergvall, N., R\"onnback, J. 2003, A\&A, 408, 887
\bibitem[\"Ostlin et al.(2021)]{O21}\"Ostlin, G., Rivera-Thorsen, T.E., Menacho, V. et al. 2021, ApJ, 912, 155
\bibitem[Papaderos et al.(1998)]{P98}Papaderos, P., Izotov, Y. I., Fricke, K. J., Thuan, T. X., Guseva, N. G., 1998, A\&A, 338, 43
\bibitem[Papaderos et al.(2002)]{P02} Papaderos, P., Izotov, Y. I., Thuan, T. X. et al. 2002 A\&A, 393, 461
\bibitem[Papaderos \& \"{O}stlin(2012)]{PO12} Papaderos, P. \& \"{O}stlin, G., 2012, A\&A, 537, A126 \tref{(PO12)}
\bibitem[Papaderos et al.(2006)]{P06}Papaderos, P., Guseva, N.G., Izotov, Y.I., Noeske, N.G., Thuan, T.X., Fricke, K.J. 2006, A\&A 457, 45
\bibitem[Papaderos et al.(2013)]{P13} Papaderos, P., Gomes, J. \& V\'{i}lchez, J. et al. 2013, A\&A, 555, L1
\bibitem[Papaderos et al.(2022)]{P22}Papaderos, P., Breda, I., Humphrey, A., Gomes, J.M., Ziegler, B.L., Pappalardo, C. 2022, A\&A. 658, A74 \tref{(P22)}
\bibitem[Papovich et al.(2001)]{Papovich01}Papovich, C., Dickinson, M. \& Ferguson, H. C. 2001, ApJ, 559, 620
\bibitem[Papovich et al.(2003)]{Papovich03}Papovich, C., Giavalisco, M., Dickinson, M., Conselice, C.J. \& Ferguson, H. C. 2003, ApJ, 598, 827
\bibitem[Papovich et al.(2005)]{Papovich05}Papovich, C., Dickinson, M., Giavalisco, M., Conselice, C.J. \& Ferguson, H. C. 2005, ApJ, 631, 101
\bibitem[Paulino-Afonso et al.(2022)]{PA22}Paulino-Afonso, A., Gonz\'alez-Gait\'an, S., Galbany, L. et al. 2022, A\&A, 662, A86
\bibitem[Peletier \& Balcells(1996)]{PelBal96}Peletier, R.F. \& Balcells, M. 1996, AJ, 111, 223
\bibitem[Pence(1976)]{Pence76}Pence, W., 1976, ApJ, 203, 39
\bibitem[P\'erez-Gonz\'alez et al.(2022)]{PG22}P\'erez-Gonz\'alez, P., Barro, G., Annunziatella, M. et al. 2022, ApJ, submitted (arXiv:2211.00045)
\bibitem[P\'erez-Montero et al.(2021)]{PM21}P\'erez-Montero, E., Amor\'in, R., S\'anchez Elmeida, J., V\'ilchez, J.M. et al. 2021, MNRAS, 504, 1237
\bibitem[Perna et al.(2020)]{Perna20}Perna, M., Arribas, S., Catalan-Torrecilla, C., et al. 2020, A\&A, 643, A139
\bibitem[Petrosian(1976)]{Petrosian76}Petrosian, V. 1976, ApJ, 209, L1
\bibitem[Poggianti(1997)]{Poggianti97}Poggianti, B.M. 1997, A\&AS, 122, 399  % K and E corrections
\bibitem[Poggianti et al.(1999)]{Poggianti99}Poggianti, B.M., Smail, I., Dressler, A. et al. 1999, ApJ 518, 576
\bibitem[Poggianti et al.(2019)]{Poggianti19}Poggianti, B.M. Gullieuszik, M., Tonnesen, S. et al. 2019, MNRAS, 482, 4466
\bibitem[Pohlen \& Trujillo(2006)]{PT06}Pohlen, M. \& Trujillo, I. 2006, A\&A, 454, 759
\bibitem[Postman \& Geller(1984)]{PG84}Postman M. \& Geller M.J., 1984, ApJ, 281, 95    % morphology-density
\bibitem[Puech et al.(2008)]{Puech08}Puech, M., Flores, H., Hammer, F. et al. 2008, A\&A 484, 173
\bibitem[Reines et al.(2010)]{Reines10}Reines, A.E., Nidever, D.L., Whelan, D.G., et al. 2010, ApJ, 708, 26
\bibitem[Rhodes et al.(2017)]{Rhodes17}Rhodes, J., Nichol, R. C., Aubourg, É., et al. 2017, ApJS, 233, 21
\bibitem[Roche et al.(2009)]{Roche09}Roche N., Bernardi M., Hyde J. 2009, MNRAS 398, 1549 %*
\bibitem[Salim et al(2018)]{Salim18}Salim, S., Boquien, M. \& Lee, Janice C. 2018, ApJ, 859, 11
\bibitem[Salim \& Narayanan(2020)]{SN20}Salim, S. \& Narayanan, D. 2020, ARA\&A 58, 529
\bibitem[Salzer et al.(1989)]{Salzer1989b}Salzer, J.J., MacAlpine, G.M. \& Boroson, T.A. 1989, ApJ Suppl. 70, 479
\bibitem[S\'anchez(2013)]{Sanchez13Metals3D}S\'anchez, S.F. 2013, in {\sl Metals in 3D: A Cosmic View from Integral Field Spectroscopy}, I. Iglesias P\'aramo, J.M V\'ilchez, P. Papaderos \& M.M. Roth (eds.), Hindawi Publishing Corporation
\bibitem[S\'anchez et al.(2012)]{Sanchez12-DR1}S\'anchez, S.F., Kennicutt, R. C., Gil de Paz, A. et al. A\&A, 538, 8
\bibitem[Sandage(1986)]{Sandage86}Sandage, A. 1986, A\&A 161, 89
\bibitem[Schaerer \& de Barros(2009)]{SdB09}Schaerer, D. \& de Barros, S. 2009, A\&A, 502, 423
\bibitem[Schaerer et al.(2022)]{Schaerer22}Schaerer, D., Marques-Chaves, R., Barrufet, L. et al. 2022, A\&A, 665, L4
\bibitem[Schweizer et al.(1990)]{Schweizer90}Schweizer F., Seitzer P., Faber S.M. et al. 1990, ApJ, 364, L33
\bibitem[Semboloni et al.(2013)]{Semboloni13}Semboloni, E., Hoekstra, H., Huang, Z. et al. 2013, MNRAS, 432, 2385
\bibitem[S\'{e}rsic(1963)]{Sersic63}S\'{e}rsic, J. L., 1963, Boletin de la Asociacion Argentina de Astronomia, vol.6, p.41
\bibitem[Silich et al.(2003)]{Silich03}Silich, S, Tenorio-Tagle, G., Mu\~noz-Tu\~no\'on, C. 2003, ApJ, 590, 791
\bibitem[Silk(1997)]{Silk97}Silk, J. 1997, ApJ, 481, 703
\bibitem[Sirressi et al.(2022)]{Sirressi22}Sirressi, M., Adamo, A., Hayes, M. et al. 2022, MNRAS, 510, 4819
\bibitem[Stasi\'nska(1984)]{Stasinska84}Stasi\'nska, G. 1984, A\&AS, 55, 15
\bibitem[Strateva et al.(2001)]{Strateva01}Strateva, I., Ivvezic, Z., Knapp, G. R., et al. 2001, AJ, 122, 1861
\bibitem[Straughn et al.(2006)]{Straughn06}Straughn, A.N., Cohen, S.H., Ryan, R.E. et al. 2016, ApJ, 639, 724
\bibitem[Struck-Marcell \& Tinsley(1978)]{SMT78}Struck-Marcell, C. \& Tinsley, B.M. 1978, ApJ, 221, 562S
\bibitem[Sturm et al.(1996)]{Sturm96}Sturm, E., Lutz, D., Genzel, R. et al. 1996, A\&A 315, L133
\bibitem[Suess et al.(2022)]{Suess22}Suess, K.A., Kriek, M., Bezanson, R. et al. 2022, ApJ, 926, 89
\bibitem[Tacchella et al.(2015)]{Tacchella15}Tacchella S. et al., 2015, Science, 348, 314
\bibitem[Tal et al.(2009)]{Tal09}Tal T., van Dokkum P.G., Nelan J., Bezanson R., 2009, AJ, 138, 1417
\bibitem[Taylor et al.(1999)]{Taylor99}Taylor, C.L., H\"uttemeister, S., Klein, U., Greve, A. 1999, A\&A, 349, 424
\bibitem[Temple et al.(2021)]{Temple21}Temple, M.J., Hewett, P.C. \& Banerji, M. 2021, MNRAS, 2021, 508, 737
\bibitem[Tenorio-Tagle et al.(2005)]{TT05}Tenorio-Tagle, G., Silich, S., Rodr\'iguez-Gonz\'alez, A., Mu\~noz-Tu\~no\'on, C. 2005, ApJ, 620, 217
\bibitem[Tenorio-Tagle et al.(2007)]{TT07}Tenorio-Tagle, G., W\"unsch, R., Silich, S., Palous, J. 2007, ApJ, 658, 1196
\bibitem[Terlevich et al.(1991)]{Terlevich91}Terlevich, R., Melnick, J., Masegosa, J. et al. 1991, A\&A Suppl., 91, 285
\bibitem[Tinsley(1968)]{Tinsley68}Tinsley, B. M. 1968, ApJ, 151, 547
\bibitem[Tolman(1930)]{Tolman30}Tolman, R.C. 1930, PNAS, 16, 511
\bibitem[Tolman(1934)]{Tolman34}Tolman, R.C. 1934, Relativity, Thermodynamics, and Cosmology (Oxford: Clarendon Press)
\bibitem[Tremonti et al.(2004)]{Tremonti04} Tremonti, C.A.,Heckman, T.M., Kauffmann, G., Brinchmann, J. et al. 2004, ApJ, 613, 898
\bibitem[Trujillo et al.(2001)]{Trujillo01}Trujillo, I., Graham, A. W. \& Caon, N. 2001a, MNRAS, 326, 869  %*
\bibitem[Trujillo et al.(2004)]{Trujillo04}Trujillo, I., Erwin, P., Asensio Ramos, A. \& Graham, A. W. 2004, AJ 127, 1917
\bibitem[Trujillo et al.(2021)]{Trujillo21}Trujillo, I., D’Onofrio, M., Zaritsky, D. et al. 2021, A\&A, 654, A40
\bibitem[Trujillo \& Bakos(2013)]{TB13}Trujillo, I. \& Bakos, J. 2013, MNRAS, 431, 1121
\bibitem[Tully \& Fisher(1977)]{TF77}Tully, R.B. \& Fisher, J.R. 1977, A\&A, 54, 661
\bibitem[Vika et al.(2014)]{Vika14}Vika, M., Bamford, S.P., H\"au\ss ler, B. \& Rojas, A.L. 2014, MNRAS 444, 3603
\bibitem[Wang et al.(2022)]{Wang22}Wang, W., Kassin, S.S., Faber, S.M., Koo, D.C. et al. 2022, ApJ, 930, 146
\bibitem[Weilbacher \& Fritze-v. Alvensleben(2001)]{WeilbacherUF01}Weilbacher, P. \& Fritze von Alvensleben, U. 2001, A\&A 373, L9
\bibitem[Weilbacher et al.(2002)]{Weilbacher02}Weilbacher, P.M., Fritze-v. Alvensleben, U., Duc, P.-A. \& Fricke, K.J. 2002, ApJ, 579, L79
\bibitem[Whitaker et al.(2011)]{Whitaker11}Whitaker, K.E., Labb\'e, I., van Dokkum, P.G. et al. 2011, ApJ, 735, 86
\bibitem[Windhorst et al.(2002)]{Windhorst02}Windhorst, R.A., Taylor, V.A., Jansen, R.A. et al. 2002, ApJ Suppl. 143, 113
\bibitem[Woo \& Ellison(2019)]{WE19}Woo, J. \& Ellison, S.L. 2019, MNRAS 487, 1928
\bibitem[Worthey et al.(1994)]{Worthey94}Worthey. G., Faber, S. M., Gonzalez J. J., Burstein, D., 1994, ApJ Suppl. 94, 687
\bibitem[Wright(2006)]{Wright06}Wright, E.L. 2006, PASP 118, 1711
\bibitem[Wuyts et al.(2012)]{Wuyts12}Wuyts, S., F\"orster Schreiber, N., Genzel, R. et al. 2012, ApJ 753, 114
\bibitem[van den Bergh(2001)]{vdBergh01}van den Bergh, S. 2001, AJ, 122, 621
\bibitem[van Zee(2000)]{vZ00}van Zee, L. 2000, AJ, 119, 2757     % UGC 5205
\bibitem[Voigt et al.(2012)]{Voigt12}Voigt, L.M., Bridle, S.L., Amara, A. et al. 2012, MNRAS, 421, 1385
\bibitem[Zackrisson et al.(2008)]{Zackrisson08}Zackrisson, E., Bergvall, N. \& Leitet, E. 2008, ApJ, 676, L9
\bibitem[Zackrisson et al.(2001)]{Zackrisson01}Zackrisson, E., Bergvall, N., Olofsson, K. \& Siebert, A. 2001, A\&A 375, 814
\bibitem[Zanella et al.(2015)]{Zanella15}Zanella, A., Daddi, E., Le Floc'h, E. et al. 2015, Nature, 521, 54
\bibitem[Zaritsky et al.(2014)]{Zaritsky14}Zaritsky, D., Courtois, H., Mu\~noz-Mateos, J.-C. et la. 2014, ApJ, 147, 134
\bibitem[Ziegler et al.(2002)]{Ziegler02}Ziegler, B.L., B\"ohm, A., Fricke, K.J. et al. 2002, ApJ, 564, L69
\end{thebibliography}

